Evolution of Star Cluster Within Galaxy using Self-consistent Hybrid Hydro/N-body Simulation

We introduce a GPU-accelerated hybrid hydro/N-body code (Enzo-N) designed to address the challenges of concurrently simulating star clusters and their parent galaxies. This task has been exceedingly challenging, primarily due to the considerable computational time required, which stems from the substantial scale difference between galaxies (~ 0.1 Mpc) and star clusters (~ pc). Yet, this significant scale separation means that particles within star clusters perceive those outside the star cluster in a semi-stationary state. By leveraging this aspect, we integrate the direct N-body code (Nbody6++GPU) into the cosmological (magneto-)hydrodynamic code (Enzo) through the utilization of the semi-stationary background acceleration approximation. We solve the dynamics of particles within star clusters using the direct N-body solver with regularization for few-body interactions, while evolving particles outside -- dark matter, gas, and stars -- using the particle-mesh gravity solver and hydrodynamic methods. We demonstrate that Enzo-N successfully simulates the co-evolution of star clusters and their parent galaxies, capturing phenomena such as core collapse of the star cluster and tidal stripping due to galactic tides. This comprehensive framework opens up new possibilities for studying the evolution of star clusters within galaxies, offering insights that were previously inaccessible.

==> 1_intro.tex <==
\section{Introduction} 

The realm of cosmological hydrodynamic simulations has marked significant progress in enhancing our comprehension of the large-scale structure and galaxy formation. On cosmological scales, dark matter-only simulations have effectively captured the evolution of the large-scale structure \citep{springel2005MNRAS.364.1105S,klypin2011ApJ...740..102K}. Furthermore, full-physics simulations, incorporating various models for astrophysical phenomena ranging from star formation to AGN feedback, have yielded realistic cosmic galaxy populations \citep{genel2014MNRAS.445..175G,nelson2018MNRAS.475..624N,springel2018MNRAS.475..676S,ni2022MNRAS.513..670N}. Zoom-in simulations have also contributed by focusing on the evolution of galaxies within the cosmological context \citep{hopkins2010MNRAS.407.1529H,kim2019ApJ...887..120K}. Moreover, they have delved into specific areas such as the formation of the first stars \citep{abel2002Sci...295...93A,yoshida2006ApJ...652....6Y} and the formation of massive black holes in the early universe \citep{regan2017NatAs...1E..75R}.
In spite of the adaptability and versatility of cosmological simulations, offering variable resolutions and targeting diverse astrophysical phenomena, none have successfully resolved the evolution of star clusters.



A star cluster is a complex dynamical system comprising approximately a million star particles, involving intricate dynamical and astrophysical phenomena, including binaries and stellar evolution \citep{2010ARA&A..48..431P}. 
The holy grail of star cluster simulation has been to perform a self-consistent collisional N-body calculation for more than a million star particles over several billion years.
The advent of direct N-body simulations has succeeded in capturing the dynamical evolution of star clusters \citep{heggie1975MNRAS.173..729H,aasrseth1999PASP..111.1333A, makino1997ApJ...480..432M,wang2015MNRAS.450.4070W, wang2016MNRAS.458.1450W}. 
Moreover, star cluster simulations have progressed to comprehensively address not only the dynamic evolution of star clusters \citep{mcmillan1990ApJ...362..522M,heggie2006MNRAS.368..677H,hurley2012MNRAS.425.2872H} but also a diverse range of astrophysical phenomena.
This includes, but is not limited to, \revision{stellar evolution} \citep{zwart2001MNRAS.321..199P, hurley2001MNRAS.323..630H,hut2003NewA....8..337H,sippel2012MNRAS.427..167S,kamlah2022MNRAS.511.4060K,kamlah2022MNRAS.516.3266K,banerjee2020A&A...639A..41B}, X-ray binaries \citep{mapelli2013MNRAS.429.2298M, spera2015MNRAS.451.4086S,ryu2016MNRAS.456..223R}, and the formation and evolution of intermediate-mass black holes \citep{zwart2002ApJ...576..899P, zwart2004Natur.428..724P, baumgardt2004ApJ...613.1133B,arca2023MNRAS.526..429A}.


Although there have been great efforts on both fronts, achieving a self-consistent full physics simulation for star clusters on a galactic scale or larger has been challenging. 
Nonetheless, there have been endeavors to integrate hydrodynamic engines into direct N-body simulations, and vice versa.
\citet{fujii2007PASJ...59.1095F} introduces a hybrid direct-tree N-body code called {\sc BRIDGE}, aiming to simultaneously resolve both star clusters and their parent galaxies. 
It employs two different time-stepping schemes for the internal motion of star clusters and all other motions, respectively. 
The internal motion of star clusters, which generally requires higher precision, is solved by the direct Hermite integrator, while other motions are calculated with a second-order Leapfrog integrator.



Despite its sophisticated implementation, {\sc BRIDGE} lacks hydrodynamics. 
On the other hand, {\sc MUSE} and its successor {\sc AMUSE} seamlessly link between different physical modules, including various hydrodynamic engines and gravity solvers \citep{zwart2009NewA...14..369P,pelupessy2013A&A...557A..84P}.
Specifically, {\sc AMUSE} encompasses a wide range of physical modules in different domains such as ph4 (Hermite N-body), Twobody (Kepler solver), MI6 (Hermite with Post-Newtonian), MESA (Stellar evolution), Gadget-2 (TreeSPH), and more.
Another hybrid hydro/N-body code presented in \citet{hubber2013MNRAS.430.1599H} combines the smoothed particle hydrodynamics (SPH) and the N-body method in order to model the collisional star cluster in a live gas background.
The SPH gas particles are integrated with the second order Leapfrog integrator, whereas the stars are integrated with the fourth order Hermite time integrator.
More recently, the ASURA project is equipped with the SPH solver, ASURA, within the BRIDGE scheme \citep{fujii2021PASJ...73.1057F}.
For the direct integration, it employs a tree direct N-body code, {\sc PeTar} \citep{wang2020MNRAS.497..536W}.




The advent of the hybrid codes enables the study of star clusters in various astrophysical environments in a more self-consistent way.
For instance, \citet{rieder2013MNRAS.436.3695R} performs a dark-matter-only simulation for the cosmological box of $(21 h^{-1}\mathrm{Mpc})^3$, and by replacing 30 dark matter particles with star clusters of 32000 particles, investigates the cosmological evolution of star clusters in the presence of cosmological tidal fields using the AMUSE framework without hydrodynamics.
The formation and evolution of massive objects, considered as potential seeds for supermassive black holes, have been investigated through processes involving gas accretion and particle-particle collisions within a dense cluster with a mass of approximately $\sim10^4\msun$ over $\sim 10^5$ Myr \citep{boekholt2018MNRAS.476..366B,reinoso2023MNRAS.521.3553R}.
\citet{wall2019ApJ...887...62W} has performed hybrid simulations, comprising magneto-hydrodynamics, collisional gravity, and star formation and evolution, to study the formation of star clusters in turbulent gas clouds of $10^3 - 10^5 \msun$ up to $20$ Myr. 


%\citet{darma2021MNRAS.506.4603D} has investigated the formation and evolution of binary star clusters for $50 \myr$ in the Milky Way and in the Large Magellanic Cloud using a multi-scale N-body simulation.
%\citep{dinnbier2020MNRAS.499..748D} implements 4th-order Herimite integrator in the Flash framework and studies the gas expulsion of star clusters.



Nevertheless, these studies face limitations in terms of system size, the breadth of physics considered, and the duration of evolution.
This is primarily attributed to the strong coupling between physical modules, particularly between hydrodynamics and collisional gravity solvers.
In order to tackle this issue, we adopt a weak coupling between the `hydro' and `nbody' parts.
Here, the `nbody' part encompasses the direct N-body solver and the regularization, while the `hydro' part includes collisionless gravity, (magneto)hydrodynamics, cosmology, and sub-resolution models.
Our {\newenzo} is a novel hybrid framework designed to facilitate robust self-consistent simulations of star clusters within their parent galaxies.
This is achieved by seamlessly integrating the direct N-body code ({\nbody}) into the (magneto-)hydrodynamic code ({\enzo}).
{\nbody} is purpose-built for simulating star clusters, utilizing a direct N-body approach, fourth-order Hermite integrator, and regularizations for few-body interactions \citep{wang2015MNRAS.450.4070W}. 
On the other hand, {\enzo} is a versatile tool addressing a broad spectrum of astrophysical problems, incorporating various physics engines such as (magneto-)hydrodynamics, PM gravity solver, gas chemistry, radiative cooling, cosmological expansion, and sub-resolution models for star formation and feedback \citep{enzo2014ApJS..211...19B}.


The hydro' and nbody' parts are connected through a weak coupling facilitated by the background acceleration, which acts as a messenger enabling communication between particles undergoing direct N-body calculations and those that do not. 
The background acceleration is computed from dark matter, gas, and stars--—entities not subject to direct N-body interactions—--on the hydro' part and transmitted to the `nbody' part. 
Subsequently, the nbody' part utilizes this semi-stationary background acceleration as the tidal field, which is updated every hydro time steps. 
The exploitation of background acceleration is justified by the considerable difference in the dynamical time scales of star clusters and galaxies, approximately $1 \myr$ and $100 \myr$, respectively.
This discrepancy results in the tidal fields of the galaxy appearing semi-stationary to the particles within star clusters.
Leveraging this, our goal in {\newenzo} is to simulate the evolution of star clusters atop a semi-stationary background potential from their parent galaxy or cosmological tidal fields for more than $100 \myr$ (up to the Hubble time). 
Throughout this process, we aim to preserve the physical integrity of the star clusters using the direct N-body solver.


%Despite the great efforts on both ends, the self-consistent full physics simulation for star clusters in a galactic scale or more has been challenging.
%\cite{passy2014ApJS..215....8P} enzo adaptive gravity

This paper is structured as follows:
In Sec. \ref{sec:method}, we provide a comprehensive description of the detailed implementation of {\newenzo}.
In Sec. \ref{sec:isolated_star_cluster}, we examine the efficacy of the direct N-body calculations in {\newenzo} by comparing it to {\nbody}. Additionally, we highlight the improved performance of {\newenzo} compared to {\enzo};
In Sec. \ref{sec:orbit}, we assess the robustness of background acceleration, comparing it to the analytic solution and {\enzo}.
In Sec. \ref{sec:agora_star_cluster}, we explore the scientific potential of {\newenzo} by simulating star clusters within their parent galaxies; 
Finally, we summarize our results in Sec. \ref{sec:summary}.



\iffalse
runaway stars or bh can alter the properties and evolution of the gas clumps or star clusters.

A numerical integration scheme for the N-body gravitational problem \citep{ahmad1973JCoPh..12..389A}\\
Investigation of SMBH formation scenario on supermassive stars (SMSs) of $10^{3}-10^{5}\msun$ via gas accretion and runaway stellar collisions in high-redshift metal-poor nuclear star clusters (NSCs) using N-body simulations. They show that star collision time-scale can as short as that of gas accretion and it is sensitive to initial conditions \citep{Das2021MNRAS.503.1051D}\\
in a massive primordial star cluster, collisions lead to SMS. Gas accretion and collision plays a role in forming SMS \citep{boekholt2018MNRAS.476..366B}\\
Merger of globular clusters, which concludes that massive clusters contribute mostly to NSC using N-body simulations. Note that they run N-body simulations for cluster mergers: https://arxiv.org/pdf/2303.18123.pdf (can't find in ads).\\
the formation of globular clusters is insensitive to star formation intensity in the host (observation) 2304.02450.\\
\citep{nagele2023arXiv230405013N} metal-enriched SMS\\
\citep{andersson2020MNRAS.494.3328A} argues the impact of runaway stars, which are kicked out of their natal gas clumps due to few-body interactions prior to the SNe, on evolution and properties of galaxy.
This highlights the necessity of inclusion of few-body physics within galaxy simulations.
\fi



==> 2_method.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{img/diagram.png}
    \caption{Overview of {\newenzo}.
   ``Enzo Particles'' encompasses entities such as dark matter, black holes, and stars, which do not play a direct role in the dynamics of star clusters.
   On the other hand, ``N-body Particles'' refers to particles, including stars and black holes, that are directly linked to the dynamics and evolution of star clusters. 
    }
    \label{fig:diagram}
\end{figure*}

\section{Numerical Method}
\label{sec:method}
In this section, we introduce {\newenzo}, a cutting-edge hybrid code that integrates a direct N-body simulation into a cosmological (magneto-)hydrodynamic code.
Through this integration, we expand the capabilities of {\nbody}, designed for simulating collisional interactions within a single or a few star clusters, to encompass galactic or cosmological scales.
Our pipeline comprises two main components: the `hydro' part and the `nbody' part. 
The hydro part, based on Enzo, handles cosmology, (magneto-)hydrodynamics, collisionless gravity, and sub-resolution physics such as radiative cooling, star formation, and black hole accretion. 
On the other hand, the nbody part is dedicated to modeling collisional gravity through the direct sum method. 
The primary role of EnzoN is to serve as the bridge connecting the hydro part and the nbody part. 
The interaction between these two components is facilitated by the use of the ``background acceleration'', which is calculated within the hydro part using the PM solver and incorporates contributions from dark matter, gas, and stars within the galaxy, excluding those in star clusters.

Fig. \ref{fig:diagram} depicts the overview of {\newenzo}.
The physical entities of {\newenzo} are categorized into two different parts: 
1. softened particles subject to particle mesh (PM) gravity solver ({\it Enzo Particles}), 
2. point mass particles subject to direct sum gravity solver that accounts for the particle-particle interaction ({\it N-body Particles}) and gas on the grids subject to hydrodynamic and PM solvers ({\it Gas}).
In the initial phase of the hydro part, we compute both the full acceleration and the background acceleration. 
In the subsequent step, the background acceleration is transmitted to the nbody part, where the dynamics of the {\it N-body Particles} is calculated using the direct sum method and regularization in addition to the background acceleration (refer to Sec. \ref{sec:method_nbody}). 
Concurrently, the hydrodynamics and subgrid physics are solved within the hydro part in parallel.
%Hereafter, background potential denotes PM gravity from both gas and smoothed particles.

\subsection{Gravito-hydrodynamic code: {\enzo}}
\label{sec:method_hydro}
{\enzo} stands as a versatile gravito-hydrodynamic computational tool crafted to address a wide spectrum of astrophysical inquiries \citep{enzo2014ApJS..211...19B}. 
Its use extends to the realms of large-scale structure formation, galaxy evolution, and the evolution of black holes. 
It boasts a rich suite of baryon physics modules encompassing stellar processes, radiative cooling, and black hole accretion. 
%\ys{details and add more?}
{\enzo}'s hydrodynamic engine relies on an Eulerian scheme on top of block-structured adaptive mesh refinement, including four different numerical hydrodynamic methods: the hydrodynamic-only piecewise parabolic method \citep{colella1984JCoPh..54..174C,bryan1995CoPhC..89..149B}, the MUSCL-like Godunov scheme \citep{vanleer1977JCoPh..23..276V,wang2008ApJS..176..467W,wang2009ApJ...696...96W}, a constrained  transport  (CT)  staggered  MHD  scheme  \citep{collins2010ApJS..186..308C}, and the second-order finite difference hydrodynamics method \citep{stone1992ApJS...80..753S,stone1992ApJS...80..791S}.
Concurrently, gravity is addressed through the implementation of the Particle Mesh solver (PM solver), along with the mesh structure. 
The collisionless particles governed by the PM solver are advanced through a single timestep using a drift-kick-drift algorithm \citep{hockney1988csup.book.....H}.
This ensures second-order accuracy even in the presence of varying time-steps due to dynamical grid structures of adaptive refinement.

\subsubsection{Time-stepping in {\enzo}}
{\enzo} adaptively integrates  the  equations, owing to the adaptive mesh-grid structure, not only in  space  but also in time.
The time step is determined on a level-by-level basis, ensuring the selection of the largest timestep that satisfies various criteria for different physical components. 
These criteria encompass hydrodynamics, acceleration, particle velocity, radiation pressure, heat conduction, and the expansion of the universe (refer to Sec. 9 in \citet{enzo2014ApJS..211...19B} for details).
For instance, the time step for hydrodynamics is given as 
\begin{equation}
    \Delta t_{\rm hydro} = \min\left(\kappa_{\rm hydro}\left(\sum_{x,y,z}\frac{c_{\rm s}+|v_{x}|}{a\Delta x}\right)^{-1}\right)_{\rm L},
\end{equation}
where $c_s$, $a$, $\Delta x$, and $\kappa$ are, respectively, the sound speed, cosmic scale factor, cell size, and a dimensionless constant for ensuring that the Courant–Freidrichs–Levy condition is always met.
Here, $\min(\cdots)_\mathrm{L}$ finds the minimum value for all cells or particles on a given level L.
In this work, we adopt $\kappa_{\rm hydro}$ of 0.3 (typically set to $0.3-0.5$).
In the case of acceleration, the time step is determined by
\begin{equation}
    \Delta t_{\rm acc} = \min\left(\sqrt{\frac{\Delta x}{|\boldsymbol{g}|}}\right)_{\rm L}.
\end{equation}
The combination of the time step and drift-kick-drift algorithm ensures second-order accuracy for gravity \citep{hockney1988csup.book.....H}.
%All grids on a given level are advanced with the same timestep. 





\subsection{Direct N-body code: {\nbody}}
\label{sec:method_nbody}

We present here descriptions of algorithms used in {\nbody} \citep{wang2015MNRAS.450.4070W}. Most methods implemented in {\nbody} are retained in {\newenzo}, except for methods that needs to commensurate with {\enzo}, such as time steps.

\subsubsection{Hermite integration with individual time steps}
\label{sec:method_hermite}

{\nbody} is a direct {\it N}-body code based on a fourth-order Hermite integration method \citep{makino1991ApJ...369..200M}. This method utilizes the lower order derivatives to obtain approximate values for higher order derivatives of each particle. Block time steps are assigned to each particle so that the quantized time step for each particle is smaller than the time step criteria. The criteria of time steps for the particles are given by

\begin{equation}
\label{eq:tcrit}
    \Delta t = \sqrt{\eta \frac{ |\mathbf{a}^{(0)}| |\mathbf{a}^{(2)}| + |\mathbf{a}^{(1)}|^{2} }{ |\mathbf{a}^{(1)}| |\mathbf{a}^{(3)}| + |\mathbf{a}^{(2)}|^{2} } },
\end{equation}
where $\Delta t$ is the criteria for time step and $\mathbf{a}^{(n)}$ is the n-th derivative of acceleration \citep{aarseth2006GReGr..38..983M}. The steps are quantized in powers of 1/2, where the unit for time step is Hénon units \citep{heggie1986LNP...267..233H}. 
The time-stepping is independently managed within the 'hydro' and 'nbody' parts. 
Communication is initiated when $n\Delta t_\mathrm{nbody} > \Delta t_\mathrm{hydro}$ for an arbitrary number of time steps $n$, where $\Delta t_\mathrm{nbody}$ is the block time step of the `nbody' part, and $\Delta t_\mathrm{hydro}$ is the finest time step of the 'hydro' part. 
During communication, the velocities and positions of N-body particles are transmitted to the 'hydro' part, and the background acceleration is sent to the 'nbody' part. 
However, in case of a mismatch between the time steps of the 'nbody' and 'hydro' parts, the positions and velocities of particles within the 'nbody' part are extrapolated to match the time step of the 'hydro' part.
The calculation in the `nbody' part resumes from the extrapolated time in blocks with quantized values of Hénon units. 
The time steps used for extrapolation are set to be equal or smaller than the time step given by Eq. \ref{eq:tcrit}. 
Furthermore, the time steps of the `nbody' part retain their consistency regardless of communication with the `hydro' part, ensuring that the physics remains unaffected. 
The detailed correspondence between {\nbody} and {\newenzo} in terms of physical results is discussed in Sec. \ref{sec:isolated_star_cluster}.



\subsubsection{Ahmad-Cohen neighbor scheme}
\label{sec:method_ac-scheme}

Direct calculation of particles up to fourth-order is computationally expensive, so {\nbody} employs a neighbor scheme described by \citep{ahmad1973JCoPh..12..389A}. In this scheme, the total force on a particle is divided into short-range ({\it irregular}) and long-range ({\it regular}) components. The irregular force is calculated from neighbor particles within a certain radius of the target particle. All the other particles are considered as contributors for regular force. The irregular force is updated at shorter intervals than the regular force. During irregular time steps, the regular force is estimated up to first-order using the derivatives calculated at regular time steps. In {\newenzo}, an additional force component from {\enzo} must be considered as well. Since the fluctuation of the background force from {\enzo} is expected to be less intensive than {\nbody}, the background force component is added to the regular force components when calculating.


\subsubsection{Regularization of close encounters}
\label{sec:method_regularization}

Accurate modeling of close encounters is crucial for the correct evolution of star clusters; 
however, handling close encounters using the Hermite scheme is both time-consuming and inaccurate.
Therefore, algorithms of \citep{KustaanheimoSCHINZELDAVENPORTSTIEFEL+1965+204+219} and \citep{mikkola1993CeMDA..57..439M} are adopted in {\nbody}.
Particles in binary or triple systems are taken out and replaced by their center of mass in the main integration code. 
The relative positions of members are calculated using regularization algorithms, while the center of mass is updated by the Hermite scheme. 



\iffalse

\subsubsection{Fourth-order Hermite Integrator}
\ys{SY: Could you summarize the fourth-order Hermite integrator as you did in the slack or something?}

\begin{itemize}
    \item Importance of time stepping
    \item  Extrapolation for Ezno, but this should not affect the physics
\end{itemize}


\ys{maybe comparison to Enzo's timestepping scheme?}


\subsubsection{KS regularization: Two-body and Three-body interaction}
\label{sec:KS}
\begin{itemize}
    \item Brief introduction of KS reg.
    \item Maybe here or in the future work, we might mention that how this scheme can be utilized for sophisticated black physics.
    \sy{well actually for treatment of black holes, I think another scheme is used.. (although some ideas for treating BH would be parallel with regularlization algorithms. )so probably it would be better to include BH in future work...}
\end{itemize}

\fi


\subsection{Center of Mass Frame}
\label{sec:method_com}
Simulating star clusters on a larger scale poses a challenge due to the hindrance caused by the peculiar or bulk motion of the star clusters, which significantly hampers computational speed. 
As discussed in Sec. \ref{sec:method_hermite}, the time-stepping in the `nbody' part is determined as a function of acceleration and its derivatives.
While the velocity dispersion of a star cluster is on the order of 10 km/s, that of a Milky-Way mased galaxy is on the order of $10^2$ km/s, indicating the relative magnitudes of self-gravity.
In the case of a star cluster situated in the spiral arms, the gravitational force exerted on the center of mass of the star cluster significantly surpasses its self-gravity.
\revision{
This may lead to issues, primarily regarding time steps.
In Eq. \ref{eq:tcrit}, we use acceleration and its derivatives to determine time steps for each particle.
However, our current setup cannot obtain higher-order derivatives for tidal accelerations from the background, potentially resulting in unphysical time steps.
This problem exacerbates when tidal accelerations that affect the motion of the center of mass dominate the accelerations of particles processed in the 'nbody' part.
}
%To prevent this, 
%This results in exceedingly small time steps in the fourth-order Hermite integrator, creating redundancy. 
To mitigate this issue, we routinely update the positions, velocities, and background acceleration of the N-body particles in the center of mass frame within the 'nbody' part, while analytically solving for the bulk motion.
\revision{This results in only non-bulk tidal gravity remaining, which is generally much weaker than the self-gravity of star clusters.}


\iffalse
\subsection{Philosophy of this framework}
\label{sec:method_philosophy}
summary of time scales? and semi-stationary background acceleration
\fi




















